GraphTheta: A Distributed Graph Neural Network Learning System With Flexible Training Strategy

Graph neural networks (GNNs) have been demonstrated as a powerful tool for analyzing non-Euclidean graph data. However, the lack of efficient distributed graph learning systems severely hinders applications of GNNs, especially when graphs are big and GNNs are relatively deep. Herein, we present GraphTheta, the first distributed and scalable graph learning system built upon vertex-centric distributed graph processing with neural network operators implemented as user-defined functions. This system supports multiple training strategies and enables efficient and scalable big-graph learning on distributed (virtual) machines with low memory. To facilitate graph convolutions, GraphTheta puts forward a new graph learning abstraction named NN-TGAR to bridge the gap between graph processing and graph deep learning. A distributed graph engine is proposed to conduct the stochastic gradient descent optimization with a hybrid-parallel execution, and a new cluster-batched training strategy is supported. We evaluate GraphTheta using several datasets with network sizes ranging from small-, modest- to large-scale. Experimental results show that GraphTheta can scale well to 1,024 workers for training an in-house developed GNN on an industry-scale Alipay dataset of 1.4 billion nodes and 4.1 billion attributed edges, with a cluster of CPU virtual machines (dockers) of small memory each (5$\sim$12GB). Moreover, GraphTheta can outperform DistDGL by up to $2.02\times$, with better scalability, and GraphLearn by up to $30.56\times$. As for model accuracy, GraphTheta is capable of learning as good GNNs as existing frameworks. To the best of our knowledge, this work presents the largest edge-attributed GNN learning task in the literature.

==> figures/Results.tex <==


%-------------------------------------------------------------------------------
\section{Experiments and Results}
%-------------------------------------------------------------------------------

\subsection{Experiment Setups}
%
\textbf{Datasets Information.}
%
We evaluate the performance of our system by training node classification models using 6 datasets.
As shown in  Table~\ref{tbl:dataset}, the network sizes vary from small-, modest-, to large-scale. 
The first five datasets including Cora, Citeseer, Pubmed, Reddit and Aamzon are publicly available and have only node attributes, without edge attributes or types.
Cora, Citeseer and Pubmed~\cite{Citationdata} are three citation networks with nodes representing documents and edges indicating citation relationship between documents.
In the three datasets, the attribute of a node is a bag-of-words vector, which is sparse and high-dimensional, while the label of the node is the category of the corresponding document.
Reddit is a post-to-post graph in which one post forms one node and two posts are linked if they are both commented by the same user.
In Reddit, a node label presents the community a post belongs to~\cite{hamilton2017inductive}.
Amazon is a co-purchasing graph, where nodes are products and two nodes are connected if purchased together.
In Amazon, node labels represent the categories of products~\cite{ClusterGCN}.

The last Alipay dataset is an industrial big graph, which contains 1.4 billion nodes and 4.1 billion attributed edges and is relatively sparse with the density of about 3.
In this dataset, nodes are users, attributes are user profiles and class labels are the financial risk levels of users.
Edges are built from a series of relations among users such as chatting, online financial cooperation, payment, and trade.
To the best of our knowledge, \todo{Alipay is the largest edge-attributed industry-scale graph ever used to test GNNs that use edge attributes in their graph convolutions in the literature.}
In our experiments, we equally split the data set into two parts, one for training and the other for testing.

\input{table_dataset}

\textbf{GNN Training Settings.}
%
\todo{We employ the node classification task as the application and use the popular GCN~\cite{kipf2016semi} model and our in-house developed GAT-E model for performance comparison.
Herein, we would like to emphasize that in these tests, our purpose is not to conclude which DL framework or GNN implementation is superior to others, but to demonstrate that GraphTheta is capable of learning GNNs as well as existing frameworks.
%Moreover, for readers' information, Appendix~\ref{appendix:gat} gives the accuracy comparison based on GAT\cite{2017GAT}
Note that although there are only node classification tasks in our tests, our system can actually support other types of tasks with moderate changes, such as revising the decoders to accommodate specific task and keeping graph embedding encoder part unchanged.}

In our tests, different datasets are configured to have varied hidden layer sizes. Specifically, hidden layer sizes are 16, 128 and 200 for the three citation networks (i.e., Cora, Citeseer and PubMed), Reddit and Amazon.
Except for Amazon, all the others have their own sub-sets for validation.
Moreover, the latter enables dropout for each layer, whereas the former does not.
In terms of global-batch, we train the model up to 1,000 epochs and select the trained model with the highest validation accuracy to test generalization performance for the latter.
With respect to mini-batch, early stop is exerted once stable convergence has reached for each dataset.
In all tests, cross-entropy loss function is used to measure convergence and prediction results are produced by feeding node embeddings to a Softmax layer.

For global-batch, we set 500 epochs for Reddit at maximum, and activate early stop as long as validation accuracy reaches stable. Meanwhile, a maximum number of 750 epochs is used for Amazon.
For mini-batch, each training step randomly chooses 1\% labeled nodes to form the initial batch for Reddit, and 0.1\% for Amazon.
This results in a batch size of 1,500 for the former and 1,710 for the latter.
We train Reddit for 600 steps and Amazon for 2,750 steps with respect to mini-batch.
Note that as Reddit (and Amazon) is a dense co-comment (and co-purchasing) network, the two-hop neighbors of only 1\% (and 0.1\%) labeled nodes almost touch 80\% (and 65\%) of all nodes.
For cluster-batch, each training step randomly chooses 1\% clusters to form the initial batch for Reddit and Amazon, where clusters are created beforehand.
% These clusters are created beforehand  and the total number is 4,300 and 8,500 for Reddit and Amazon respectively. 
In addition, cluster-batch applies the same early stop strategy as mini-batch.

%
\subsection{Accuracy Assessment}
%
\subsubsection{Evaluation on Public Datasets.}
On the public datasets, we train a two-layer GCN model~\cite{kipf2016semi} using our system and compare the performance with the state-of-the-art counterparts, including a TensorFlow-based implementation (TF-GCN) from~\cite{kipf2016semi}, a DGL-based one (DGL), Cluster-GCN and two neighbor-sampling-based ones: FastGCN and VR-GCN. 

\textbf{Comparison with non-sampling-based methods.}
First, we compare our system with TF-GCN, DGL and Cluster-GCN to demonstrate that our system can achieve highly competitive or superior generalization performance on the same datasets and models, even without using sampling.
Table~\ref{tbl:result_small} shows the performance comparison on the three small-scale citation networks, i.e., Cora, Citeseer and PubMed~\cite{Citationdata}.
For DGL and Cluster-GCN, we resue the results presented in \cite{wang2019deep} and ~\cite{ClusterGCN}, respectively, instead of evaluating them.
This is because both of them did not completely expose their hyper-parameters and pose challenges for result reproduction.
Both GraphTheta and TF-GCN use the same set of hyper-parameter values, including learning rate, dropout keep probability, regularization coefficient, and batch size, as proposed in~\cite{kipf2016semi}, and train the model 300 steps for mini-batch.
From the table, global-batch yields the best accuracy for each dataset, with an exception that its performance is neck-by-neck with that of mini-batch on Citeseer.
Mini-batch also outperforms both DGL and TF-GCN for each case.

Due to the small sizes of the three networks, we run one worker of 1 GB memory, \todo{in our Kubernetes CPU cluster}, to train each of them.
In terms of the average time per epoch/step, our method obtains on the Cora, Citeseer and PubMed datasets of 0.18 (0.21) seconds, 0.85 (0.24) seconds, and 0.3 (0.27) seconds respectively with respect to the global-batch (mini-batch) training. \todo{For Cora, its mini-batch is slower than global-batch because of two reasons. One is that Cora is too small and thereby the runtime per epoch/step is very short, and the other is that in each training step, mini-batch does some extra preparation work like neighborhood subgraph identification whose runtime is considerable for small datasets.}

\input{table_result}
\input{table_alipay}

\textbf{Comparison with sampling-based methods.}
%
Second, we compare our implementations (without sampling) with FastGCN, VR-GCN and Cluster-GCN on the two modest-scale datasets: Reddit and Amazon.
FastGCN employs importance neighbor sampling, VR-GCN adopts variance reduction, whereas Cluster-GCN does not use sampling same as GraphTheta.
Both FastGCN and VR-GCN train models in a mini-batched manner.
Table~\ref{tbl:result_middle} gives the test accuracy of each experiment.
For FastGCN, VR-GCN and Cluster-GCN, we directly use the results from their corresponding publications.
Note that the performance of FastGCN on Amazon is unavailable, and the algorithm will not participate in the performance evaluation with respect to Amazon.

On both datasets, global-batch yields the best accuracy, while mini-batch performs the worst with cluster-batch in between.
In terms of Reddit, FastGCN is inferior to VR-GCN, while Cluster-GCN is superior to VR-GCN.
However, with respect to Amazon, Cluster-GCN becomes slightly worse than VR-GCN.
It is worth mentioning that the relatively lower performance of our cluster-batch may be caused by multiple factors, e.g. number of clusters,  cluster batching,  and the quality of graph partitioning.
In sum, based on the aforementioned observations, it is reasonable to draw the conclusion that sampling-based training methods are not always better than non-sampling-based ones.

We train the two networks by launching 600 and 200 workers, each of which has a memory size of 4 GB, respectively.
For Reddit, our method obtains an average time per epoch/step of 75.42 seconds, 57.88 seconds and 35.81 seconds in terms of global-batch, mini-batch and cluster-batch.
For Amazon, the corresponding results are 43.11 seconds, 32.62 seconds and 19.00 seconds, respectively.
%
\subsubsection{Evaluation on Alipay dataset}
\label{sub_section:alipay}
%
In this test, we use our in-house developed GAT-E model, a graph attention network that incorporates edge attributes to attention computation along with node attributes.
GAT-E is a simplified version of the GIPA~\cite{zheng2021gipa} algorithm and is trained on Alipay dataset with all of the three training strategies.

Table~\ref{tbl:result_large} shows the accuracy on Alipay dataset.
We run 400 epochs for global-batch, and 3,000 steps for all the others.
Cluster-batch performs the best, while mini-batch outperforms global-batch, in terms of both F1 score and accuracy.
In terms of convergence speed in the same distributed environment, we can observe that cluster-batch converges the fastest. The second fastest method is global-batch, and the third one is mini-batch. 
Specifically, the overall training time of 1,024 workers is 30 hours for global-batch, 36 hours for mini-batch, and 26 hours for cluster-batch, and the peak memory footprint per worker is 12~GB, 5~GB and 6~GB respectively.
%
%
\subsection{Scalability Assessment}
%
\subsubsection{Comparison of Different Training Strategies}
\label{sec:alipay_scale}
%
\input{fig_scale}
%
We evaluate the capability of strong scaling to big graphs of GraphTheta with respect to the number of workers using Alipay dataset.
Each worker is equipped with one computing thread and runs in a Linux CPU Docker.
Due to the large memory footprint of Alipay dataset, we start from 256 workers and use this performance as the baseline.

\todo{
Figures.~\ref{fig:gb_scale}, \ref{fig:cb_scale} and \ref{fig:mb_scale} illustrate the speedup results in the function of the number of workers for global-batch, cluster-batch and mini-batch respectively.
From the figures, we can see that each of three training strategies can scale to 1024 workers, and the speedups for the forward, backward and full training steps are consistent in terms of the scaling size for each training strategy.
This can be explained by our observation that the neural network functions are usually compute-intensive and thus lead to better computation and communication overlap, significantly lowering the impact of communication.
By investigating the speedups of the three training strategies, it can be observed that global-batch has the best scalability, followed by cluster-batch and mini-batch in decreasing order.
This is because ($i$) global-batch has relatively balanced workloads among workers, since all nodes in the graph participate in the computation simultaneously, and ($ii$) cluster-batch has better data locality within distributed machines, resulting in less inter-machine communication than mini-batch.
}

\todo{In the following we will analyze the speedups and parallel efficiency gained as the number of workers varies.
For global-batch, by increasing the number of workers from 256 to 512, the forward runs $1.66\times$ faster, the backward $1.75\times$ faster, and the full training step $1.72\times$ faster.
Furthermore, when increasing the number of works further to 1,024, the speedups become $2.81$, $3.21$ and $3.09$ times respectively.
In terms of parallel efficiency, the forward achieves $83\%$ (and $70\%$),  backward of $87\%$ (and $80\%$), and  full training steps of $86\%$ (and $77\%$) by using 512 workers (and 1,024 workers).
}

\todo{
In terms of cluster-batch, when moving from 256 to 512 (and 1024) workers, the speedup is 1.70 (and 1.75) for the forward, 1.74 (and 2.45) for the backward, and 1.52 (and 1.80) for the full training step.
In this case, the corresponding parallel efficiency becomes $85\%$ (and $44\%$) for the forward, $87\%$ (and $61\%$ for the backward, and $76\%$ (and $45\%$) for the full training step.
}

\todo{
With respect to mini-batch, compared to the baseline performance with 256 workers, the speedup and parallel efficiency with 512 workers is 1.83 and $91\%$ for the forward, 1.77 and $88\%$ for the backward, and 1.71 and $86\%$ for the full training step, respectively.
Meanwhile, the corresponding values with 1024 workers are 1.84 and $46\%$ for the forward, 2.85 and $71\%$ for the backward, and 2.23 and $56\%$ for the full training step, respectively.
}

\subsubsection{Comparison with DistDGL}
%
\todo{In this section, we will compare with DistDGL~\cite{zheng2020distdgl, zheng2021distributed} in terms of scalability by training GCN model on the Reddit dataset.
In this test, we disable node sampling for the DistDGL node data loader for fair comparison.
We exclude Dorylus~\cite{thorpe2021dorylus} and ROC~\cite{jia2020improving} from this comparison for the following reasons. 
Firstly, Dorylus is based on AWS Lambda and cannot run in our Kubernetes cluster.
Secondly, Dorylus performs graph operations in distributed graph servers and conducts neural network operations by Lambda threads. However, it still needs to load all neighbors of given targets nodes into Lambda threads. This is same as DistDGL.
Thirdly, Dorylus runs slower than DGL (non-sampling) on Reddit as shown in its own paper.
Finally, ROC requires each graph server to load the entire graph into memory and thus does not match the objective of our tests for fully distributed graphs.
}

\todo{In this test, we launch GraphTheta and DistDGL to synchronously train the aforementioned GNN model with mini-batch on a cluster of 8 computers with 64 CPU cores and 300 GB RAM each.
We set to use 4 cores for each worker/trainer and keep the overall batch size unchanged (i.e. the batch size per worker/trainer times the number of workers/trainers is equal to a constant value).
Figure~\ref{fig:distdgl_scale} illustrates the comparison of scalability between GraphTheta and DistDGL in the function of number of workers/trainers on Reddit. 
From the figure, we can see that as the number of workers/trainers increases, GraphTheta gets superior to DistDGL. More specifically, with 8 trainers, DistDGL yields a speedup of 29.4 relative to GraphTheta.
However, when moving to 128 trainers, DistDGL becomes slower than GraphTheta that runs $1.32\times$ faster than the former.
This phenomenon is due to the good scalability of GraphTheta, as demonstrated in Section~\ref{sec:alipay_scale}.
Nevertheless, we admit that compared to DistDGL using coarse-grained sparse tensor operations, the performance of our implementations based on fine-grained vertex programs still have a large room for improvement.
}
%
\subsection{Effect of Graph Partitioning Methods}
\label{result:partition}
%
\input{fig_partition}
%
\todo{In this section, we will evaluate the effect of the following two graph partitioning methods: \texttt{vertex-cut} and \texttt{1D-edge partition}, on the execution speeds of the three training strategies using Amazon dataset.
\texttt{vertex-cut} is a 2D-grid partitioning method, which targets to evenly distribute edges to all workers.
Given an edge, \texttt{vertex-cut} determines the worker it is assigned to by computing the hash values from the source and destination nodes of the edge.
\texttt{1D-edge partition} aims to evenly distribute source (or destination) nodes to all workers.
Given an edge, \texttt{1D-edge partition} determines its destination worker by computing a hash value from the source (or destination) node.
In our implementation, we compute the hash value from the source node, which is also the master node, but allow for users to configure to use the destination.
\texttt{vertex-cut} has the advantage of addressing the highly skewed node degree distribution problem, while \texttt{1D-edge partition} leads to better edge locality for the perspective of source (or destination) nodes.}

\todo{In GraphTheta, we set \texttt{1D-edge partition} as the default partitioning method, based on the following two considerations.
On one hand,  the use of edge attention and edge embedding has been becoming more and more popular in GNNs~\cite{wu2020comprehensive,zhang2020deep,chaudhari2021attentive}.
With \texttt{vertex-cut}, the edges of a given master node are likely distributed onto multiple workers.
In this case, the computation of edge attention and edge embedding will incur considerable extra communication. 
On the contrary, \texttt{1D-edge partition} always places a master node and all of its edges together in the same worker.
This way, we can compute the edge attention and edge embedding for the master node locally, with no need of extra communication.
On the other hand, in practice we observe that \texttt{vertex-cut} usually has higher peak memory footprint than \texttt{1D-edge partition}.
Taking the tests on Amazon as an example, the peak memory of \texttt{vertex-cut} is about 20\% larger than that of \texttt{1D-edge partition} on average.
Nevertheless, users can still specify their preferred partitioning method at the runtime.}

\todo{Figures~\ref{fig:partition_gb_amazon}, \ref{fig:partition_cb_amazon} and \ref{fig:partition_mb_amazon} show the normalized average runtimes of the forward, the backward and the full epoch steps, respectively in terms of global-batch,  cluster-batch and mini-batch.
The normalization uses the corresponding runtime of \texttt{1D-edge partition} as the baseline.
From the figures, \texttt{vertex-cut} has the better performance than \texttt{1D-edge partition} for global-batch and mini-batch, and is inferior to the latter for cluster-batch.
Based on these observations, we would like to make the following suggestion. If there is sufficient memory in distributed machines, we recommend users trying \texttt{vertex-cut} first in an optimistic manner. Otherwise, \texttt{1D-edge partition} is supposed to be in preference to \texttt{vertex-cut}.}
%


==> figures/fig_partition.tex <==
%
%
\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figures/fig_distdgl_scale.pdf}
\caption{Scalibility comparison between GraphTheta and DistDGL on Reddit.}
\label{fig:distdgl_scale}
\end{figure}
%
%
\begin{figure*}[t!]
\centering
\subfigure[Global-batch]{
\includegraphics[width=0.31\linewidth]{figures/partition_gb_amazon.pdf}
\label{fig:partition_gb_amazon}
}
%
\subfigure[Cluster-batch]{
\includegraphics[width=0.31\linewidth]{figures/partition_cb_amazon.pdf}
\label{fig:partition_cb_amazon}
}
%
%
\subfigure[Mini-batch]{
\includegraphics[width=0.31\linewidth]{figures/partition_mb_amazon.pdf}
\label{fig:partition_mb_amazon}
}
%
\caption{Performance comparison between vertex-cut and 1D-edge partititon methods on Amazon for each training strategy.}
\label{fig:partition_amazon}
\end{figure*}
%

